Monte-Carlo radiative transfer simulation of the circumstellar disk of the Herbig Ae star HD 144432

Studies of pre-transitional disks, with a gap region between the inner infrared-emitting region and the outer disk, are important to improving our understanding of disk evolution and planet formation. Previous infrared interferometric observations have shown hints of a gap region in the protoplanetary disk around the Herbig Ae star HD~144432. We study the dust distribution around this star with two-dimensional radiative transfer modeling. We compare the model predictions obtained via the Monte-Carlo radiative transfer code RADMC-3D with infrared interferometric observations and the {\SED} of HD~144432. The best-fit model that we found consists of an inner optically thin component at $0.21\enDash0.32~\AU$ and an optically thick outer disk at $1.4\enDash10~\AU$. We also found an alternative model in which the inner sub-AU region consists of an optically thin and an optically thick component. Our modeling suggests an optically thin component exists in the inner sub-AU region, although an optically thick component may coexist in the same region. Our modeling also suggests a gap-like discontinuity in the disk of HD~144432.

==> tabular.model.1comp_curved_dataset1.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    $R_\mathrm{in}$ $[\AU]$
    & $0.1\enDash0.5$
    & $5$
    & $0.334$
    \\
    $R_\mathrm{out}$ $[\AU]$
    & $2\enDash10$
    & $3$
    & $4.47$
    \\
    $h_\mathrm{in}$
    & $0.01\enDash0.06$
    & $6$
    & $0.02$
    \\
    $p_h$
    & $0.1\enDash0.7$
    & $7$
    & $0.4$
    \\
    $f_\mathrm{curve}$
    & $5\enDash20$
    & $4$
    & $5$
    \\
    \hline
    $\pSigma$
    & $-1$
    & $-$
    & $-1$
    \\
    $\TauMidPlane$
    & $10^{ 4}$
    & $-$
    & $10^{ 4}$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $0.1$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{1,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}

\renewcommand{\TabularParameterDescription}{
  The listed parameters are:
  $f_\mathrm{curve}=\textrm{curvature of the inner rim}$,
  other parameters are same as in Fig.1.
}



==> tabular.model.1comp_curved_dataset2.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    $R_\mathrm{in}$ $[\AU]$
    & $0.1\enDash0.5$
    & $5$
    & $0.224$
    \\
    $R_\mathrm{out}$ $[\AU]$
    & $2\enDash10$
    & $3$
    & $4.47$
    \\
    $h_\mathrm{in}$
    & $0.01\enDash0.06$
    & $6$
    & $0.05$
    \\
    $p_h$
    & $0.1\enDash0.7$
    & $7$
    & $0.1$
    \\
    $f_\mathrm{curve}$
    & $5\enDash20$
    & $4$
    & $5$
    \\
    \hline
    $\pSigma$
    & $-1$
    & $-$
    & $-1$
    \\
    $\TauMidPlane$
    & $10^{ 4}$
    & $-$
    & $10^{ 4}$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $0.1$
    & $-$
    & $0.1$
    \\
    \hline
    $\chi^2_\mathrm{2,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}



==> tabular.model.1comp_dataset1.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    $R_\mathrm{in}$ $[\AU]$
    & $0.05\enDash0.6$
    & $7$
    & $0.262$
    \\
    $R_\mathrm{out}$ $[\AU]$
    & $1\enDash100$
    & $5$
    & $31.6$
    \\
    $h_\mathrm{in}$
    & $0.01\enDash0.10$
    & $10$
    & $0.03$
    \\
    $p_h$
    & $0.0\enDash0.8$
    & $9$
    & $0.3$
    \\
    \hline
    $\pSigma$
    & $-1$
    & $-$
    & $-1$
    \\
    $\TauMidPlane$
    & $10^{ 4}$
    & $-$
    & $10^{ 4}$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{1,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}

\renewcommand{\TabularParameterDescription}{
  The listed parameters are:
  $R_\mathrm{in}=\textrm{inner radius of the disk}$,
  $R_\mathrm{out}=\textrm{outer radius of the disk}$,
  $h_\mathrm{in}=\textrm{scale height at inner radius}$,
  $p_{h}=\textrm{scale-height power-law index}$,
  $p_{\Sigma}=\textrm{surface-density power-law index}$,
  $\TauMidPlane=\textrm{midplane optical depth at 2 }\mum$,
  $f_\mathrm{small}=\textrm{fraction of small grains in the dust}$,
  $f_\mathrm{carbon}=\textrm{fraction of carbon in the dust}$.
}




==> tabular.model.1comp_dataset2.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    $R_\mathrm{in}$ $[\AU]$
    & $0.05\enDash0.6$
    & $7$
    & $0.262$
    \\
    $R_\mathrm{out}$ $[\AU]$
    & $1\enDash100$
    & $5$
    & $3.16$
    \\
    $h_\mathrm{in}$
    & $0.01\enDash0.10$
    & $10$
    & $0.08$
    \\
    $p_h$
    & $0.0\enDash0.8$
    & $9$
    & $0.0$
    \\
    \hline
    $\pSigma$
    & $-1$
    & $-$
    & $-1$
    \\
    $\TauMidPlane$
    & $10^{ 4}$
    & $-$
    & $10^{ 4}$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{2,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}



==> tabular.model.1comp_secondary_dataset1.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    $R_\mathrm{in}$ $[\AU]$
    & $0.262$
    & $-$
    & $0.262$
    \\
    $R_\mathrm{out}$ $[\AU]$
    & $31.6$
    & $-$
    & $31.6$
    \\
    $h_\mathrm{in}$
    & $0.03$
    & $-$
    & $0.03$
    \\
    $p_h$
    & $0.3$
    & $-$
    & $0.3$
    \\
    \hline
    $\pSigma$
    & $-2\enDash0$
    & $5$
    & $0$
    \\
    $\TauMidPlane$
    & $10^{1}\enDash10^{6}$
    & $6$
    & $10^{3}$
    \\
    $f_\mathrm{carbon}$
    & $0.0\enDash1.0$
    & $6$
    & $0.4$
    \\
    $f_\mathrm{small}$
    & $0,0.01,0.1,0.5,1$
    & $5$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{1,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}

\renewcommand{\TabularParameterDescription}{}



==> tabular.model.1comp_shadowed_dataset1.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    $R_\mathrm{in}$ $[\AU]$
    & $0.1\enDash0.5$
    & $5$
    & $0.334$
    \\
    $W_\mathrm{rim}$
    & $0.2,~0.5,~1.0$
    & $3$
    & $0.2$
    \\
    $h_\mathrm{puff}$ $[\AU]$
    & $0.01\enDash0.05$
    & $5$
    & $0.02$
    \\
    $R_\mathrm{out}$ $[\AU]$
    & $10$
    & $-$
    & $10$
    \\
    $h_\mathrm{in}$
    & $0.01\enDash0.10$
    & $10$
    & $0.02$
    \\
    $p_h$
    & $0.0\enDash0.6$
    & $7$
    & $0.5$
    \\
    \hline
    $\pSigma$
    & $-1$
    & $-$
    & $-1$
    \\
    $M_\mathrm{dust}$
    & $10^{-6}$
    & $-$
    & $10^{-6}$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{1,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}

\renewcommand{\TabularParameterDescription}{
  The listed parameters are:
  $W_\mathrm{rim}=\textrm{non-dimensional width of the inner rim}$,
  $h_\mathrm{puff}=\textrm{additional scale height of the rim}$,
  other parameters are same as in Fig.1.
}



==> tabular.model.1comp_shadowed_dataset2.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    $R_\mathrm{in}$ $[\AU]$
    & $0.1\enDash0.5$
    & $5$
    & $0.224$
    \\
    $W_\mathrm{rim}$
    & $0.2,~0.5,~1.0$
    & $3$
    & $0.5$
    \\
    $h_\mathrm{puff}$ $[\AU]$
    & $0.01\enDash0.05$
    & $5$
    & $0.05$
    \\
    $R_\mathrm{out}$ $[\AU]$
    & $10$
    & $-$
    & $10$
    \\
    $h_\mathrm{in}$
    & $0.01\enDash0.10$
    & $10$
    & $0.02$
    \\
    $p_h$
    & $0.0\enDash0.6$
    & $7$
    & $0.6$
    \\
    \hline
    $\pSigma$
    & $-1$
    & $-$
    & $-1$
    \\
    $M_\mathrm{dust}$
    & $10^{-6}$
    & $-$
    & $10^{-6}$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{1,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}



==> tabular.model.2comp_ThinNull_Rin_Wring_dataset2.tex <==

\renewcommand{\TabularContent}{ 
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    Inner disk
    \\
    $R_\mathrm{in}$ $[\AU]$
    & $0.05\enDash0.6$
    & 21
    & $0.119$
    \\
    $W_\mathrm{ring}$
    & $0.1\enDash3.0$
    & $21$
    & $3.0$
    \\
    $\pSigma$
    & $0$
    & $-$
    & $0 $
    \\
    $h_\mathrm{in}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $\tau$
    & $0.39$
    & $-$
    & $0.39$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{2,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}


==> tabular.model.2comp_ThinNull_dataset2.tex <==

\renewcommand{\TabularContent}{ 
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    Inner disk
    \\
    $R_\mathrm{in}$ $[\AU]$
    & $0.05\enDash0.6$
    & 21
    & $0.173$
    \\
    $W_\mathrm{ring}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    $\pSigma$
    & $0$
    & $-$
    & $0 $
    \\
    $h_\mathrm{in}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $\tau$
    & $0.1 \enDash3.0$
    & 21
    & $0.33$
    \\
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{2,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}



==> tabular.model.2comp_ThinThick_SubMM_dataset0.tex <==

\renewcommand{\TabularContent}{ 
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    \multicolumn{4}{l}{
      Component 1 (inner disk)
    }
    \\
    $R_\mathrm{in,1}$ $[\AU]$
    & $0.212$
    & $-$
    & $0.212$
    \\
    $W_\mathrm{ring,1}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $p_{\Sigma,1}$
    & $0$
    & $-$
    & $0$
    \\
    $h_\mathrm{in,1}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $\tau_1$
    & $0.1 \enDash 0.2$
    & $6$
    & $0.14$
    \\
    \hline
    \multicolumn{4}{l}{
      Component 2 (outer disk)
    }
    \\
    $ R_\mathrm{in,2}   [\AU]$
    & $1.0\enDash1.5$
    & $6  $
    & $1.4$ 
    \\
    $R_\mathrm{out,2}$ $[\AU]$
    & $10$
    & $- $
    & $10$
    \\
    $p_{\Sigma,2}$
    & $-1 $ 
    & $-$
    & $-1 $ 
    \\
    $h_\mathrm{in,2}$
    & $0.02\enDash0.04$
    & $5$
    & $0.035$
    \\
    $p_{h,2}$
    & $0.3\enDash0.5$
    & $3 $
    & $0.3$
    \\
    $M_\mathrm{dust,2}$
    & $10^{-4}$
    & $-$
    & $10^{-4}$       
    \\
    \hline
    $f_\mathrm{carbon}$
    & $0.1$
    & $-$
    & $0.1$
    \\
    $f_\mathrm{small}$
    & $0.1\enDash1.0$
    & $5$
    & $0.18$
    \\
    \hline
    $\chi^2_\mathrm{0,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}

\renewcommand{\TabularParameterDescription}{
  The listed parameters are similar to those in Fig. 4.
}



==> tabular.model.2comp_ThinThick_dataset1.tex <==

\renewcommand{\TabularContent}{ 
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    \multicolumn{4}{l}{
      Component 1 (inner disk)
    }
    \\
    $R_\mathrm{in,1}$ $[\AU]$
    & $0.15\enDash0.3$
    & 5
    & $0.212$
    \\
    $W_\mathrm{ring,1}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $p_{\Sigma,1}$
    & $0$
    & $-$
    & $0$
    \\
    $h_\mathrm{in,1}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $\tau_1$
    & $0.15\enDash0.7$
    & 5
    & $0.15$
    \\
    \hline
    \multicolumn{4}{l}{
      Component 2 (outer disk)
    }
    \\
    $W_\mathrm{gap}   [\AU]$
    & $0.0\enDash2.0$
    & $5  $
    & $0.5$ 
    \\
    $R_\mathrm{out,2}$ $[\AU]$
    & $10$
    & $- $
    & $10$
    \\
    $p_{\Sigma,2}$
    & $-1 $ 
    & $-$
    & $-1 $ 
    \\
    $h_\mathrm{in,2}$
    & $0.02\enDash0.06$
    & $5 $
    & $0.02$
    \\
    $p_{h,2}$
    & $0.1\enDash0.5$
    & $5 $
    & $0.5$
    \\
    $M_\mathrm{dust,2}$
    & $10^{-6}$
    & $-$
    & $10^{-6}$       
    \\
    \hline
    $f_\mathrm{carbon}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $f_\mathrm{small}$
    & $1.0$
    & $-$
    & $1.0$
    \\
    \hline
    $\chi^2_\mathrm{1,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}

\renewcommand{\TabularParameterDescription}{
  The listed parameters are:
  $W_\mathrm{ring,1}=(R_\mathrm{out,1}-R_\mathrm{in,1}) / R_\mathrm{in,1}$
  (relative radial width of the inner component),
  $W_\mathrm{gap}=R_\mathrm{in,2}-R_\mathrm{out,1}$
  (radial width of the gap),
  $R_{\mathrm{in},i}=\textrm{inner radius of component }i$,
  $R_{\mathrm{out},i}=\textrm{outer radius of component }i$,
  $h_{\mathrm{in},i}=\textrm{scale height of cpmponent $i$ at its inner radius}$,
  $p_{h,i}=\textrm{scale-height power-law index of cpmponent $i$}$,
  $p_{\Sigma,i}=\textrm{surface-density power-law index of cpmponent $i$}$,
  $\tau_i = \textrm{midplane optical depth of component $i$ at }2~\mum$,
  $M_{\mathrm{dust},i} = \textrm{dust mass of component $i$}$.
}



==> tabular.model.3comp_DoubleThick_SubMM_dataset0.tex <==

\renewcommand{\TabularContent}{
  \begin{tabular}{ccccc}
    \hline
    \hline
    \HeadLineForModelTabular
    \\
    \hline
    \multicolumn{4}{l}{Component 1
      (inner optically thin disk)
    }
    \\
    $R_\mathrm{in,1}$ $[\AU]$
    & $0.1\enDash0.15$
    & $6$
    & $0.15 $
    \\
    $W_\mathrm{ring,1}$
    & $2.0$
    & $-$
    & $2.0$
    \\
    $p_{\Sigma,1}$
    & $0$
    & $-$
    & $0$
    \\
    $h_\mathrm{in,1}$
    & $0.5$
    & $-$
    & $0.5$
    \\
    $\tau_1$
    & $0.1 \enDash0.2$
    & 6
    & $0.12 $
    \\
    \hline
    \multicolumn{4}{l}{Component 3
      (inner optically thick disk)
    }
    \\
    $R_\mathrm{in,3}/R_\mathrm{in,1}$
    & $1$
    & $-$
    & $1$
    \\
    $R_\mathrm{out,3}/R_\mathrm{in,1}$
    & $1.25 $
    & $-$
    & $1.25 $
    \\
    $p_{\Sigma,3}$
    & $-1 $ 
    & $- $
    & $-1 $ 
    \\
    $h_\mathrm{in,3}$
    & $0.005$
    & $- $
    & $0.005$
    \\
    $p_{h,3}$
    & $0.0$
    & $- $
    & $0.0$
    \\
    $\tau_\mathrm{3}$
    & $10^{4}$
    & $-$
    & $10^{4}$       
    \\
    \hline
    \multicolumn{4}{l}{
      Component 2 (outer disk)
    }
    \\
    $R_\mathrm{in,2}$ $[\AU]$
    & $1.4  $
    & $-$
    & $1.4   $
    \\
    $R_\mathrm{out,2}$ $[\AU]$
    & $10$
    & $-$
    & $10$
    \\
    $p_{\Sigma,2}$
    & $-1 $ 
    & $-$
    & $-1 $ 
    \\
    $h_\mathrm{in,2}$
    & $0.03\enDash0.045$
    & $7 $
    & $0.0375$
    \\
    $p_{h,2}$
    & $0.3$
    & $- $
    & $0.3$
    \\
    $M_\mathrm{dust,2}$
    & $10^{-4}$
    & $-$
    & $10^{-4}$       
    \\
    \hline
    $f_\mathrm{carbon}$
    & $0.1$
    & $-$
    & $0.1$
    \\
    $f_\mathrm{small}$
    & $0.1\enDash0.5$
    & $5$
    & $0.4 $
    \\
    \hline
    $\chi^2_\mathrm{0,red}$
    &
    &
    & \BestChiSquare
    \\
    \hline
  \end{tabular}
}


